Semantic Reasoning with Differentiable Graph Transformations

This paper introduces a differentiable semantic reasoner, where rules are presented as a relevant set of graph transformations. These rules can be written manually or inferred by a set of facts and goals presented as a training set. While the internal representation uses embeddings in a latent space, each rule can be expressed as a set of predicates conforming to a subset of Description Logic.

==> acro_list.tex <==
\begin{acronym}[Bi-LSTM]
    \acro{Bi-GCN}{Bi\--directional Graph Convolutional Network}
    \acro{Bi-LSTM}{Bi\--directional Long Short-Term Memory}
    \acro{LSTM}{Long Short-Term Memory}
    \acro{GCN}{Graph Convolutional Network}
    \acro{GRU}{Gated Recurrent Unit}
    \acro{LSTM}{Long Short-Term Memory}
    \acro{NER}{Named Entity Recognition}
    \acro{NLP}{Natural Language Processing}
    \acro{PoS}{Part\--of\--Speech}
    \acro{RNN}{Recurrent Neural Network}
    \acro{EL}{Entity Linking}
    \acro{NED}{Named Entity Disambiguation}
    \acro{WSD}{Word Sense Disambiguation}
\end{acronym}

